Clones, closed categories, and combinatory logic

We give an exposition of the semantics of the simply-typed lambda-calculus, and its linear and ordered variants, using multi-ary structures. We define universal properties for multicategories, and use these to derive familiar rules for products, tensors, and exponentials. Finally we explain how to recover both the category-theoretic syntactic model and its semantic interpretation from the multi-ary framework. We then use these ideas to study the semantic interpretation of combinatory logic and the simply-typed lambda-calculus without products. We introduce extensional SK-clones and show these are sound and complete for both combinatory logic with extensional weak equality and the simply-typed lambda-calculus without products. We then show such SK-clones are equivalent to a variant of closed categories called SK-categories, so the simply-typed lambda-calculus without products is the internal language of SK-categories. As a corollary, we deduce that SK-categories have the same relationship to cartesian monoidal categories that closed categories have to monoidal categories.

==> sec-conclusion.tex <==
%We have seen three main things. First, that by using category-theoretic ideas to isolate the correct universal properties for multi-ary structures 
%	(as in \Cref{sec:universal-properties-for-multicategories}), 
%one can `read off' the syntax, semantic interpretation and syntactic category for several important type-formers in the (linear) simply-typed $\uplambda$-calculus. 
%%
%We spelled this out for products in 	
%		\Cref{sec:recovering-the-semantics-for-cartesian},
%but similar remarks hold for each of the languages considered.
%%
%In each case, the core technical result is that  we can factor the usual semantic interpretation through the multi-ary one as in~(\ref{eq:factoring-free-properties-schematically}).
%
%Second, we introduced multi-ary semantic models for combinatory logic and showed they coincide with those for simply-typed $\uplambda$-calculus
%	(\Cref{res:main-theorem-for-clones}).
%%	
%Finally, we characterised a categorical structure that is sound and complete for simply-typed $\uplambda$-calculus without products (\Cref{res:factoring-adjunction-for-closed-clones}).
%
%
%\paragraph*{Related work.}
%%
%The insight that multi-ary structures are natural models of syntax goes back to Lambek~(\cite{Lambek1969,Lambek1989}), and clone aficionados will likely be unsurprised by the development of \Cref{sec:cartesian-clones,sec:closed-clones,sec:cc-clones}.
%%
%Indeed, the core idea of using multi-ary structures has been exploited in various special cases: the identification of linear $\uplambda$-calculus with certain multicategories is due to Hyland~\&~de Paiva~\cite{Hyland1993}, while Jacobs essentially defines closed clones for modelling $\uplambda$-calculus in~\cite{Jacobs1992}. 
%%
%More recently, the multi-ary point of view is an important part of Hyland's recent recasting of the theory of the untyped $\uplambda$-calculus~(\cite{Hyland2014,Hyland2015}); similar ideas, generalised to the 2-dimensional setting, were crucial for the soundness and completeness results of~(\cite{LICS2019,mythesis}).
%%
%An even more general framework for syntax, allowing multi-ary domains and codomains, is provided by Shulman's recent work with polycategories~\cite{Shulman2023}.
%%
%Clones have also played an important role in the 
%	`algebraic syntax'
%programme of Fiore and collaborators initiated in~\cite{Fiore1999} (see~\eg~\cite{Arkor2020,Arkor2021}).
%
%%Alternative approaches to modelling syntax, which also give models capable of modelling closed structure without products, include Jacobs' fibrational techniques~\cite{Jacobs1992} and Pitts' example of a syntactic model in~\cite[\S4.4]{Pitts2000}.
%
%\paragraph*{Future work.}
%%
%The connection between SK-categories and closed categories remains to be explored. 
%%
%This includes defining a version of closed categories which does not rely on a unit object, which may well correspond to some form of combinatory logic 
%	(as in~\eg~\cite[p.~255]{Bimbo2012}).
%%	
%Alternatively, it ought to be possible to axiomatise SK-categories in a manner similar to cartesian multicategories, by adding in duplication and deletion operations.
%
%From the syntactic perspective, it would be interesting to identify classes of languages---including those with effects---for which the binding operations can be replaced by combinators 
%	(\cf~\Cref{res:main-theorem-for-clones}), 
%and ask whether these have corresponding unary models.
%%
%Some aspects have been explored (\eg~\cite{Lafont1987,Hasegawa2023}), but it remains unclear to what extent $\stlc$ is a special case.
%%
%It also remains to be seen whether the category-theoretic perspective of SK-clones sheds new light on the traditional approach modelling combinatory logic with combinatory algebras.

